Mixed Nash Equilibria in the Adversarial Examples Game

This paper tackles the problem of adversarial examples from a game theoretic point of view. We study the open question of the existence of mixed Nash equilibria in the zero-sum game formed by the attacker and the classifier. While previous works usually allow only one player to use randomized strategies, we show the necessity of considering randomization for both the classifier and the attacker. We demonstrate that this game has no duality gap, meaning that it always admits approximate Nash equilibria. We also provide the first optimization algorithms to learn a mixture of classifiers that approximately realizes the value of this game, \emph{i.e.} procedures to build an optimally robust randomized classifier.

==> sections/section1draft.tex <==
\section{Introduction}

Adversarial examples~\citep{biggio2013evasion,Szegedy2013IntriguingPO} are one of the most dizzling problems in machine learning: state of the art classifiers are sensitive to imperceptible perturbations of their inputs that make them fail. Last years, research have concentrated on proposing new defense methods~\citep{madry2017towards,moosavi2019robustness,KolterRandomizedSmoothing} and building more and more sophisticated attacks~\citep{goodfellow2014explaining,kurakin2016adversarial,carlini2017adversarial,croce2020reliable}. So far, most defense strategies proved to be vulnerable to these new attacks or are computationally intractable. Nonetheless, a recent line of research argued that randomized classifiers could help countering adversarial attacks~\citep{pruningDefenseICLR2018,Xie2017MitigatingAE,pinot2019theoretical,NIPS2019_8443}. Along this line, \cite{pinot2020randomization} demonstrated, using game theory, that randomized classifiers are indeed more robust than deterministic ones against regularized adversaries. It is however worth noting that none of the previous works investigated the scenario where the adversary also uses randomized strategies. In this paper, we tackle this issue by analyzing the adversarial example game in the setting where both the classifier and the attacker use randomization. To motivate this study, let us discuss the following example.


%If randomization does help defending against standard (deterministic) adversaries 


%Adversarial examples~\citep{biggio2013evasion,Szegedy2013IntriguingPO} are one of the most dizzling problems in machine learning: state of the art classifiers are sensitive to imperceptible perturbations of their inputs that cause classifiers to completely fail. Last years, research have concentrated on building more and more sophisticated attacks~\citep{goodfellow2014explaining,kurakin2016adversarial,carlini2017adversarial}, on proposing new defense methods~\citep{madry2017towards,moosavi2019robustness}, but also on understanding the nature of adversarial attacks~\citep{pydi2019adversarial,pmlr-v97-dohmatob19a}. So far, this phenomenon is still misunderstood and raises important questions of security in many fields as autonomous driving CITE, face recognition CITE, recommender systems~\citep{garcelon2020adversarial} etc. In the working line on defenses, it is often argued that  randomized classifiers could help being more robust against adversarial attacks. Some former works have studied adversarial examples in the light of optimal transportation and game theory~\cite{pinot2020randomization,} but it is still an open problem to study the equilbria of the adversarial examples game in a randomized setting. In this paper tackle this problem by analyzing theoretically the equilibria of randomized strategies for both classifiers and the attacker in the adversarial example game.%In this paper, we propose to study the equilibria of ensemble methods in the adversarial setting.

\begin{figure}[t]
    \centering
\includegraphics[width=0.95\columnwidth]{Images/Drawing-Intro-Mixte-Nash.pdf}    \caption{On left: deterministic classifiers ($f_1$ on top, $f_2$ on the bottom) for whose, the blue point can always be attacked. On right: a randomized classifier, where the attacker has a probability $1/2$ of failing, regardless of the attack it selects.}
    \label{fig:motivating_ex}
\end{figure}

\paragraph{A motivating example.} Consider the binary classification task illustrated in Figure~\ref{fig:motivating_ex}. We assume that all input-output pairs $(X,Y)$ are sampled from a distribution $\PP$ defined as
$$ 
\PP\left(Y =\pm 1\right)=1/2 \ \mbox{ and }\left\{
    \begin{array}{ll}
        \PP\left(X=0 \mid Y=-1\right) = 1 \\
        \PP\left(X= \pm 1 \mid Y=1\right) = 1/2 
    \end{array}
\right.
$$
Given access to $\PP$, the adversary aims to maximize the expected risk, but can only move each point by at most $1$ on the real line. In this context, we study two classifiers: $f_1(x) = 1/2-x$ and $f_2(x)=x-1/2$\footnote{$(X,Y) \sim \PP$ is missclassified by $f_i$ if and only if $f_i(X)Y \leq 0$}. Both $f_1$ and $f_2$ have a standard risk of $1/4$. In the presence of an adversary, the risk (\emph{a.k.a.} the adversarial risk) increases to $1$. Here, using a randomized classifier can make the system more robust. Consider for example $f$ where $f=f_1$ w.p. $1/2$ and $f_2$ otherwise. The standard risk of $f$ remains $1/4$ but its adversarial risk is $3/4<1$. Indeed, when attacking $f$, any adversary will have to choose between moving points from $0$ to $1$ or to $-1$. Either way, the attack only works half of the time; hence an overall adversarial risk of $3/4$. Furthermore, if $f$ knows the strategy the adversary is planning to use, it can always update the probability it gives to $f_1$ and $f_2$ to get a better (possibly deterministic) defense. For example, if the adversary chooses to move all points from $0$ to $1$ (which is an optimal strategy), the classifier can set $f=f_1$ w.p. $1$ to retrieve a risk of $1/2$ instead of $3/4$. 

Now, what happens if the adversary can use randomized strategies, meaning that for each point it can flip a coin before deciding where to move? In this case, the adversary could for examples decide to send points from $0$ to $1$ w.p. $1/2$ and to $-1$ otherwise. This strategy is still optimal with an adversarial risk of $3/4$ but now the classifier cannot use its knowledge of the adversary's strategy to lower the risk. We are in a state where neither the adversary nor the classifier can benefit from unilaterally changing its strategy. In the game theoretical terminology, this state is called a Mixed Nash equilibrium. Previous works studying adversarial examples from the scope of game theory investigated the existence of Mixed Nash equilibria in restricted settings where the adversary can by reducted to a set of parameters~\citep{7533509,DBLP:journals/corr/abs-1906-02816,bose2021adversarial}. But, as pointed out in \cite{pinot2020randomization} and \cite{pydi2019adversarial}, studying the existence of a Mixed Nash equilibrium in a more general framework is a challenging open problem. In the present paper we tackle the following question.

\textbf{Q:} Is it always possible to reach a Mixed Nash equilibrium in the adversarial example game when both the adversary and the classifier can use randomized strategies?

\begin{enumerate}
    \item why a randomized attacker? cf example
    \item in a rand/rand case, what is the nature of the problem? 
    \item duality gap du jeu deterministe pour le classifieur-> illustre le fait quil faille randomisé. est-il necessaire -> oui cf exps
\end{enumerate}

%\textbf{A1:} this paper, we answer positively to this question. After having extended the notion of attacks to randomized attacks, we define a general adversarial example game where both the attacker and the classifier are randomized. We, then, show that the duality gap for this game is actually $0$. 

%\paragraph{A motivating example.} Le consider the simple following classification task on $X\in\mathbb{R}$ to label $Y\in\{-1,1\}$. Let assume the distribution $\PP$: $\PP(Y = 1)=\PP(Y = -1)=1/2$. Conditionally to $Y=1$, $X$ always equals $0$; and conditionally to $Y=-1$, $X=1$ with probability $1/2$ and $-1$ otherwise. The distribution is described in Figure~\ref{fig:motivating_ex}. We assume that an attacker can move every point by a distance at most $1$ with the goal to maximize the expected risk. Consider two classifier: $f_1(x) = 1/2-x$ and $f_2(x) =x-1/2$. An example $(X,Y)$ is misclassified by $f_i$ if and only $Yf_i(X)\leq 0$.  Then for $i=1,2$, the standard risk equals $1/4$ and the adversarial risk equals $1$. If we define the randomized classifier $f$ such that $f=f_1$ with probability $1/2$ and $f=f_2$ with probability $1/2$,  the standard risk of $f$ is $1/4$ and the adversarial risk is $3/4<1$. There is a gain to randomize the classifier in this context. Indeed, the best strategy for the attacker is to attack randomly $f_1$ or $f_2$ with equal probabilities when $X$ equals $0$.  If he does not do so, for instance he always attacks $f_1$, the optimal classifier against this attack is $f_2$ which is deterministic. Then to reach a Nash equilibrium, i.e. a strategy where neither the attacker or the classifier gains by changing unilaterally its own strategy, the attacker and the classifier need to play randomized strategies. 
%\begin{figure}[ht]
%    \centering
%\includegraphics[width=\columnwidth]{Images/Drawing-Intro-Mixte-Nash.pdf}    \caption{Motivating example: on left, deterministic classifiers for whose, the blue point can always be attacked. On right, randomized classifier, where the attacker might fail since on fooling the blue point, since whatever attack he makes, he has a probability $1/2$ of failing.}
%    \label{fig:motivating_ex}
%\end{figure}





%\textbf{Q2:} Although we show there is no duality gap for the adversarial game, is it possible to learn the optimal randomized classifier?

%\textbf{A2:} We treat this question when the hypothesis class of classifiers is finite: we derive two algorithms with theoretical guarantees to find the optimal mixture of classifiers. The first one, inspired from DUCHI, enjoys XX rate. The second is inspired by the literature on entropic regularization, and enjoys better convergence rates but leads to an approximate solution. 

%This yet simple example raises interesting fundamental questions with regards to adversarial examples: 

%\textbf{Q1:} Is it always possible to reach an equilibrium in a setting where both the attacker and the classifier are randomized?

%\textbf{A1:} this paper, we answer positively to this question. After having extended the notion of attacks to randomized attacks, we define a general adversarial example game where both the attacker and the classifier are randomized. We, then, show that the duality gap for this game is actually $0$. 

%\textbf{Q2:} Although we show there is no duality gap for the adversarial game, is it possible to learn the optimal randomized classifier?

%\textbf{A2:} We treat this question when the hypothesis class of classifiers is finite: we derive two algorithms with theoretical guarantees to find the optimal mixture of classifiers. The first one, inspired from DUCHI, enjoys XX rate. The second is inspired by the literature on entropic regularization, and enjoys better convergence rates but leads to an approximate solution. 
%Every Bayes optimal classifier have a $0$ natural risk, but the its adversarial risk equals to $1$.
